On the Variance of the Adaptive Learning Rate and Beyond

The learning rate warmup heuristic achieves remarkable success in stabilizing training, accelerating convergence and improving generalization for adaptive stochastic optimization algorithms like RMSprop and Adam. Here, we study its mechanism in details. Pursuing the theory behind warmup, we identify a problem of the adaptive learning rate (i.e., it has problematically large variance in the early stage), suggest warmup works as a variance reduction technique, and provide both empirical and theoretical evidence to verify our hypothesis. We further propose RAdam, a new variant of Adam, by introducing a term to rectify the variance of the adaptive learning rate. Extensive experimental results on image classification, language modeling, and neural machine translation verify our intuition and demonstrate the effectiveness and robustness of our proposed method. All implementations are available at: https://github.com/LiyuanLucasLiu/RAdam.

==> 3ana.tex <==
% \section{Variance of Adaptive Rate}

% % In this section, we first analyze the variance of adaptive learning rates, then introduce the empirical results that support our hypothesis -- it is the noise of the adaptive learning rate in the early stage causes the convergence problems.
% In this section, we first analyze the variance of adaptive learning rates, then introduce the empirical results that support our hypothesis -- \emph{Due to the lack of samples in the early stage, the adaptive learning rate has undesirably large variance and can cause convergence issues}.

% To begin with, we first analyze a special case.
% When $t = 1$, we have $\psi(g_1) = \sqrt{\frac{1}{g_i^2}}$. 
% In this paper, we view $\{g_1, \cdots, g_t\}$ as i.i.d. random variables drawn from a Normal distribution $\cN(0, \sigma^2)$.
% % Now, let's move to the special case of $t = 1$. 
% % Since $g_1 \sim \gN(0, \sigma^2)$
% Therefore, $\frac{1}{g_i^2}$ is subject to the scaled inverse chi-squared distribution, $\sics(1, \frac{1}{\sigma^2})$.
% It is easy to find that 
% $\Var[\sqrt{\frac{1}{g_i^2}}] \propto \int_0^{\infty} x^{-1} e^{-x} dx$, which is divergent. 
% It means that, the adaptive ratio can be undesirable large in the first stage of learning.
% % or cause convergence problems. 
% At the same time, setting a small learning rate at the early stage can reduce variance (since $\Var[\alpha x] = \alpha^2\Var[x]$) thus alleviating this problem.
% Therefore, we suggest that the large variance of the adaptive learning rate in the early stage can cause convergence problems.
% % In the following of this section, we first analyze the variance of adaptive learning rates, then introduce the empirical results that supports our hypothesis.

% \subsection{Analysis of Adaptive Learning Rate Variance}
% As mentioned before, Adam uses the exponential moving average to calculate the adaptive learning rate. 
% Assume $\{g_1, \cdots, g_t\}$ are i.i.d., their exponential moving average has a larger variance than their average. 
% Also, in the early stage ($t$ is small), the difference of the exponential weights of $\{g_1, \cdots, g_t\}$ is relative small (up to $1 - \beta_2^{t-1}$).
% Therefore, for ease of analysis, we approximate the moving average as the simple average, \ie, $\psi(g_1, \cdots, g_t) \approx \sqrt{\frac{t}{\sum_{i=1}^t g_i^2}}$ (further analysis on this approximation is conducted in Section~\ref{subsec:sma-ema}). 
% Now, we proceed to its variance analysis. 

% Since $g_i \sim \gN(0, \sigma^2)$, we have $\frac{t}{\sum_{i=1}^t g_i^2} \sim \sics(t, \frac{1}{\sigma^2})$. 
% Therefore, we have:
% \begin{equation}
% \E[\frac{t}{\sum_{i=1}^t g_i^2}] = \frac{t}{(t - 2) \sigma^2} \;(\forall t > 2)
% \quad\mbox{and}\quad
% \Var[\frac{t}{\sum_{i=1}^t g_i^2}] = \frac{2 t^2}{(t - 2)^2 (t - 4) \sigma^4} \;(\forall t > 4).
% \label{eqn:inv-chi-sq}
% \end{equation}

% The analytic form of $\Var[\sqrt{\frac{t}{\sum_{i=1}^t g_i^2}}]$ is derived as Equation~\ref{eqn:analytic-sqrt-var} (in Section~\ref{subsec:approx}).
% Since its calculation is complicated and not numerical stable, we use the following approximation, which is observed to have a high precision in our simulation experiments (discussions are elaborated in Section~\ref{subsec:approx}). 
% Specifically, approximating $\sqrt{x}$ to the first order~\citep{wolter2007taylor}, we have: 
% \begin{equation}
% \sqrt{x} \approx \sqrt{\E[x]} + \frac{1}{2\sqrt{\E[x]}}(x - \E[x])
% \quad\mbox{and}\quad
% \Var[\sqrt{x}] \approx \frac{\Var[x]}{4\E[x]}
% \label{eqn:sqrt-var}
% \end{equation}
% Combining Equation~\ref{eqn:inv-chi-sq} and \ref{eqn:sqrt-var}, we have:
% \begin{equation}
% \Var[\sqrt{\frac{t}{\sum_{i=1}^t g_i^2}}] \approx \frac{t}{2(t - 2) (t - 4) \sigma^2}.
% \label{eqn:variance_appro}
% \end{equation}
% It indicates that, due to the lack of samples (small $t$), in the early stage of training, the variance of the adaptive learning rate is substantially larger than the late stage.
% For example, the variance at $t = 5$ is over $100$ times larger than the variance at $t = 500$ (as in Figure~\ref{fig:var_approx}).
% In the next section, we further design controlled experiments to verify that the large variance is the cause of the convergence problems, and warmup works as a variance reduction technique.

% % \begin{figure}[t]
% % \centering
% % \begin{subfigure}[b]{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{fig/ppl.pdf}
% %     \caption{\,}
% % \end{subfigure}%
% % \begin{subfigure}[b]{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{fig/loss.pdf}
% %     \caption{\,}
% % \end{subfigure}
% % \caption{Training of Transformers on the De-En IWSLT'14 dataset. (a) Training perplexity in the first 50k gradient updates. (b) Training loss in the first 50k gradient updates.}
% %     \label{fig:eps2k}
% % \end{figure}

% \subsection{Warmup as Variance Reduction}
% In this section, we design controlled experiments to verify our hypothesis that it is the large variance of the adaptive learning rate causes the convergence issue. 
% Particularly, we design two variants of Adam: Adam-2k and Adam-eps, make comparisons to Adam with warmup and the vanilla Adam (without warmup) on the IWSLT'14 German to English dataset~\citep{cettolo2014report}. 
% In the first two thousand iterations of Adam-2k, only its exponential moving 2nd moments are updated, while its exponential moving average and parameters are fixed\footnote{Different from the previous work~\cite{gotmare2018a}, all parameters and all first moments are frozen during the first two thousand iterations.}; other than this, it follows the original Adam algorithms. 
% To compare with others, its iterations are indexed from -1999 instead of 1.
% As in Figure~\ref{fig:eps2k}, we observe that, after getting these additional two thousand samples to estimate its second moments, Adam avoids the convergence problem met by the vanilla-Adam. 
% Also, comparing Figure~\ref{fig:histogram_2} and \ref{fig:histogram_3}, getting enough samples prevents the gradient distribution from being distorted. 
% These observations verify that, it is the lack of enough samples causes the convergence issue. 

% To further verify our hypothesis, we try to demonstrate that the convergence problem can be avoided by reducing the variance of the adaptive learning rate.
% % To reduce the variance of the adaptive learning rate, a straight forward way is to increase the value of $\epsilon$ in $\hat{\psi}(g_1, \cdots, g_t) = \frac{\sqrt{1-\beta_2^t}}{\epsilon + \sqrt{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i}g_i^2}}$.
% A straight forward way to reduce the variance is to increase the value of $\epsilon$ in $\hat{\psi}(g_1, \cdots, g_t) = \frac{\sqrt{1-\beta_2^t}}{\epsilon + \sqrt{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i}g_i^2}}$.
% Actually, if we assume $\hat{\psi}(.)$ is subject to the uniform distribution, its variance equals to $\frac{1}{12 \epsilon^2}$.
% Therefore, we design an additional variants of the Vanilla-Adam, Adam-eps, which sets $\epsilon$ from a negligible value ($1\times 10^{-8}$) to a non-negligible value ($1\times 10^{-4}$).
% Its performance is also summarized in Figure~\ref{fig:eps2k}. 
% We observe that it avoids the serious convergence problem met by vanilla-Adam and verifies that the convergence problem can be alleviated by reducing the variance of the adaptive learning rate. 
% Besides, similar to Adam-2k, it prevents the gradient distribution distortion (as shown in Figure~\ref{fig:histogram_3}). 
% However, it results in worse performance comparing to Adam-2k or Adam-warmup. 
% We conjecture this is because large $\epsilon$ distorts the original design of Adam, i.e., updates are not uniformly scaled. 
% % As a brief summary, we introduce both theoretical analysis and empirical evidence supports that the adaptive learning rate has undesirably large variance in the first stage of training, and can cause convergence problems. 
% In the next section, we try to fix this issue by rectifying the variance of the adaptive learning rate. 

% \begin{figure}[t]
% \centering
%     \includegraphics[width=\textwidth]{fig/histogram_3.pdf}
% \caption{The histogram of the absolute value of gradients (on a log scale) during the training of Transformers on the De-En IWSLT' 14 dataset. }
% \label{fig:histogram_3}
% \end{figure}


==> 4fix.tex <==
% % !TEX encoding = UTF-8
% % !TEX Root = 0_main.tex
% \section{Rectified Adaptive Learning Rate}

% % In this section, we introduce our design of the variance calibration term.%, then move to improve Adam by ``centering'' its 2rd moment.

% % \subsection{Variance Calibration}
% In this section, we first derive an approximation to the variance of the moving average, then design a rectification term to address the undesirably large variance in the early stage. 

% \subsection{Variance Rectification}
% % In the proof of Theorem~\ref{theorem: variance_mono}, Equation~\ref{eqn:analytic-sqrt-var} gives the analytic form of $\Var[\psi]$, while $\nu$ is the degree of freedoms. 
% In the previous section, Equation~\ref{eqn:analytic-sqrt-var} gives the analytic form of $\Var[\psi]$, where $\nu$ is the degree of freedoms. 
% Here, we first provide an estimation of $\nu$, then derive a reliable and concise approximation.
% % of $\Var[\psi]$.

% As the exponential moving average (EMA) is widely used in eccomincs, it is usually interpretted as an approximation to the simple moving average (SMA)~\citep{nau2014forecasting}, \ie, 
% % We first approximate the exponential moving average (EMA) with the simple moving average (SMA), which accords to the scaled inverse chi-square distribution, \ie, 
% \begin{equation}
% % \label{eqn:ema_sma}
% \frac{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i}g_i^2}{1-\beta_2^t} \approx \frac{\sum_{i = 1}^{f(t, \beta_2)} g_{t+1-i}^2}{f(t, \beta_2)}.
% \end{equation}
% where $f(t, \beta_2)$ is the length of the SMA which allows the SMA has the same ``center of mass'' with the EMA.
% In other words, $f(t, \beta_2)$ satisfies:
% $$
% \frac{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i} (t+1-i)}{1-\beta_2^t} = \frac{\sum_{i = 1}^{f(t, \beta_2)} (t+1-i)}{f(t, \beta_2)}.
% $$
% Simplifies the above equation, we have:
% $$
% \frac{1}{1-\beta_2} - \frac{t  \beta_2^t}{1 - \beta_2^t}= \frac{f(t, \beta_2)+1}{2}
% \quad\mbox{and}\quad 
% f(t, \beta_2) = \frac{2}{1 - \beta_2} - 1 - \frac{2 t \beta_2^t}{1 - \beta_2^t}.
% $$
% At the same time, $\frac{\sum_{i = 1}^{f(t, \beta_2)} g_{t+1-i}^2}{f(t, \beta_2)}$ accords to the scaled inverse chi-square distribution with $f(t, \beta_2)$ degrees of freedoms. 
% Thus,
% % \begin{equation*}
%     $
%     \frac{f(t, \beta_2)}{\sum_{i = 1}^{f(t, \beta_2)} g_{t+1-i}^2} \sim \sics(f(t, \beta_2), \frac{1}{\sigma^2})
%     $
%     % \quad\mbox{is an approximation of }\quad
%     is an approximation to
%     $
%     \frac{1-\beta_2^t}{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i}g_i^2} \sim \sics(\nu, \frac{1}{\sigma^2}).
%     $
% % \end{equation*}
% Therefore, we treat $f(t, \beta_2)$ as an estimation of $\nu$. 
% For ease of notation, we mark $f(t, \beta_2)$ as $\nu_t$. Also, we record $\frac{2}{1 - \beta_2} - 1$ as $\nu_\infty$ (maximum length of the approximated SMA), due to the inequality $f(t, \beta_2) \leq \lim_{t \to \infty} f(t, \beta_2) = \frac{2}{1 - \beta_2} - 1$.

% In order to assure the adaptive factor has consistent variance, we use the following term to rectify the variance of $\nu_t$ to be the variance of $\nu_\infty$: 
% \begin{equation}
% r_t = \sqrt{\frac{\Var[\psi(.)]|_{\nu = \nu_t}}{\Var[\psi(.)]|_{\nu = \nu_\infty}}} = \sqrt{\frac{\frac{\nu_t}{\nu_t-2} - \frac{\nu_t \,2^{2\nu_t - 5}}{\pi}\gB(\frac{\nu_t-1}{2}, \frac{\nu_t-1}{2})^2}{\frac{\nu_\infty}{\nu_\infty-2} - \frac{\nu_\infty \,2^{2\nu_\infty - 5}}{\pi}\gB(\frac{\nu_\infty-1}{2}, \frac{\nu_\infty-1}{2})^2}}.
% \label{eqn:analytic-rectification}
% \end{equation}
% However, Equation~\ref{eqn:analytic-rectification} is not numerical stable and cannot be calculated efficiently. 
% Therefore, we try to derive a reliable and concise approximation to Equation~\ref{eqn:analytic-sqrt-var}.
% Specifically, approximating $\sqrt{\psi^2(.)}$ to the first order~\citep{wolter2007taylor}, we have: 
% \begin{equation}
% \sqrt{\psi^2(.)} \approx \sqrt{\E[\psi^2(.)]} + \frac{1}{2\sqrt{\E[\psi^2(.)]}}(\psi^2(.) - \E[\psi^2(.)])
% \quad\mbox{and}\quad
% \Var[\psi(.)] \approx \frac{\Var[\psi^2(.)]}{4\E[\psi^2(.)]}
% % \label{eqn:sqrt-var}
% \end{equation}
% Since $\psi^2(.) \sim \sics(\nu_t, \frac{1}{\sigma^2})$, we have:
% \begin{equation}
% \Var[\sqrt{\psi(.)}] \approx \frac{\nu_t}{2(\nu_t - 2) (\nu_t - 4) \sigma^2}.
% \label{eqn:variance_appro}
% \end{equation}
% We conduct simulation experiments to examine Equation~\ref{eqn:variance_appro} and find it is a reliable approximation to Equation~\ref{eqn:analytic-sqrt-var}. 
% Therefore, we rewrite Equation~\ref{eqn:analytic-rectification} as: 
% \begin{equation}
% r_t = \sqrt{\frac{(\nu_t - 4)(\nu_t - 2)\nu_\infty}{(\nu_\infty - 4)(\nu_\infty - 2)\nu_t}}.
% \end{equation}

% \subsection{RAdam}
% Applying our rectification term to Adam, our final algorithm is summarized in Algorithm~\ref{algo:cadam}. 
% Specifically, when the length of the approximated SMA is less or equal than 4, the variance of the adaptive learning rate is intractable and the adaptive learning rate is disabled.
% Otherwise, we will calculate the variance rectification term and update parameters with the adaptive learning rate.
% We notice that $r_t$ has a similar form with the heuristic ``warmup'' (using small learning rates in the first few epochs), which verifies our intuition that ``warmup'' works as a variance reduction technique. 


% % Based on Equation~\ref{eqn:variance_appro} and \ref{eqn:ema_sma}, we have
% % \begin{equation}
% % \Var[\sqrt{\frac{1-\beta_2^t}{(1 - \beta_2)\sum_{i = 1}^t \beta_2^{t-i}g_i^2}}]
% % \approx \Var[\sqrt{\frac{l_t}{\sum_{i=1}^{l_t} g_i^2}}]
% % \approx \frac{l_t}{2(l_t - 2)(l_t - 4)\sigma^2}.
% % \label{eqn:variance_appro_appro}
% % \end{equation}
% % In order to assure the adaptive factor has consistent variance, we design a calibration term to adjust the variance of $l_t$ to the variance for $l_\infty$: 
% % In order to assure the adaptive factor has consistent variance, we design the following term to rectify the variance of $l_t$ to be the variance of $l_\infty$: 
% % \begin{equation}
% % c_t = \sqrt{\frac{(l_t - 4)(l_t - 2)l_\infty}{(l_\infty - 4)(l_\infty - 2)l_t}}.
% % \end{equation}

% % the raw moving average (since the bias-corrected moving average has a larger variance). 

% % \subsection{Moving Variance based Adaptive Gradient}

% % As mentioned by Adam, the second moment works in a similar way with variance. 
% % Specifically, since $\Var[x] = \E[x^2] - \E[x]^2$, for parameters with the same $\E[g]$, the ones with larger variance would have larger second moment. 
% % Here, we propose to replace the moving average of second momentum with the moving variance. 
% % Specifically, our final algorithm is summarized in Algorithm~\ref{algo:cadam}. 

% \begin{algorithm}[t]
% \DontPrintSemicolon
% \KwIn{$\{\alpha_t\}_{t = 1}^T$: step size, 
% $\{\beta_1, \beta_2\}$: decay rate to calculate moving average and moving 2nd moment, \newline
% $\theta_0$: initial parameter, $f(\theta)$: stochastic objective function.}
% \KwOut{$\theta_t$: resulting parameters}
% $m_0 \gets 0$ (Initialize moving average)\;
% $v_0 \gets 0$ (Initialize moving variance)\;
% $l_\infty \gets 2/(1 - \beta_2) - 1$ (Compute the maximum length of the approximated SMA)\;
% \While{$t = \{1, \cdots, T\}$}{
%     $g_t \gets \Delta_{\theta} f_t(\theta_{t - 1})$ (Calculate gradients w.r.t. stochastic objective at timestep t)\;
%     $v_t \gets \beta_2 v_{t - 1} + (1 - \beta_2) g_t^2$ (Update exponential moving 2nd moment)\;
%     $m_t \gets \beta_1 m_{t - 1} + (1 - \beta_1) g_t$ (Update exponential moving average)\;
%     $\widehat{m_t} \gets m_t / (1 - \beta_1^t)$ (Compute bias-corrected moving average)\;
%     $l_t \gets l_\infty - 2t\beta_2^t/(1 - \beta_2^t)$(Compute the length of the approximated SMA)\;
%     \uIf{the variance is tractable, \ie, $l_t > 4$}{
%         $\widehat{v_t} \gets \sqrt{v_t / (1 - \beta_2^{t})}$ (Compute bias-corrected moving 2nd moment)\;
%         $r_t \gets \sqrt{\frac{(l_t - 4)(l_t - 2)l_\infty}{(l_\infty - 4)(l_\infty - 2)l_t}}$ (Compute the variance rectification term)\;
%         $\theta_t \gets \theta_{t-1} - \alpha_t r_t \widehat{m_t} / \widehat{v_t}$ (Update parameters with adaptive momentum)\;
%     }
%     \Else{
%         $\theta_t \gets \theta_{t-1} - \alpha_t \widehat{m_t}$ (Update parameters with un-adapted momentum)\;
%     }
% }
% \Return{$\theta_T$}
% \caption{Rectified Adam. All operations are element-wise. }
% \label{algo:cadam}
% \end{algorithm}


==> 5converge.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex
% \section{Convergence Analysis}


==> 6exp.tex <==
% % !TEX encoding = UTF-8
% % !TEX Root = 0_main.tex
% \section{Experiments}

% To empirically evaluate our proposed method, we conduct experiments with different neural networks, including CNNs, LSTMs and Transformers on both Vision tasks and NLP tasks. 
% Specifically, we first discuss the performance of CAdam on neural machine translation, on which the state-of-the-art employs Adam with ``warmup''.
% Then, we will move to the typical optimization benchmarks to evaluate the effectiveness of our method. 
% % \subsection{Transformer on Neural Machine Translation}
% % We conduct experiments on IWSLT14 De-En dataset.
% % \begin{table}[htb!]
% %     \centering
% %     \begin{tabular}{c|c|c|c|c}
% %          \multirow{2}{*}{Method} &  \multicolumn{2}{c|}{IWSLT DE-EN}& \multicolumn{2}{c}{IWSLT EN-DE}\\
% %          \cline{2-5}
% %           & ppl & GLUE  & ppl & GLUE \\
% %          \hline
% %          Adam-warmup   &  & $34.66 \pm 0.014$ &  & \\
% %          CAdam-9995   &  & $34.76 \pm 0.003$ &  &\\
% %         %  CAdam-999-warmup   &  &  &  &\\
         
% %     \end{tabular}
% %     \caption{GLUE score on Neural Machine Translation}
% %     \label{tab:nmt}
% % \end{table}

% \subsection{Transformer on Neural Machine Translation}
% We conduct experiments on IWSLT14 De-En dataset.
% \begin{table}[htb!]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          Method & IWSLT DE-EN & IWSLT EN-DE & WMT16 EN-DE \\
%          \hline
%          Adam-warmup   & $34.66 \pm 0.014$ & $28.56 \pm 0.067$ & $26.93$\\
%          CAdam-9995   & $34.76 \pm 0.003$ & $28.48 \pm 0.054$ & $27.27$\\
%         %  CAdam-999-warmup   &  &  &  &\\
         
%     \end{tabular}
%     \caption{BLEU score on Neural Machine Translation}
%     \label{tab:nmt}
% \end{table}
% % \xiaodl{Tab 1. BLEU?}
% \subsection{LSTM on Language Modeling}


% \subsection{Convolutional Neural Neetwork on Cifar10 and ImageNet}
% We conduct experiments on Cifar10, Cifar100, and IMageNet (ILSVRC2012) datasets.

% \begin{table}[htb!]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          Method &  Cifar10 & Cifar100 & ImageNet\\
%          \hline
%          Adam   &  &  & \\
%          CAdam   &  &  & \\
         
%     \end{tabular}
%     \caption{Accuracy on Image Classification}
%     \label{tab:image_cls}
% \end{table}


% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/train_loss.pdf}
%     \caption{\,}
% \end{subfigure}%
% \begin{subfigure}[b]{0.54\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/test_acc.pdf}
%     \caption{\,}
% \end{subfigure}
% \caption{Training of ResNet-18 on the cifa10 dataset. (a) Training loss. (b) Test accuracy.}
%     \label{fig:cifa10}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=\textwidth]{fig/cifa10_lr.pdf}
% \caption{Performance on Cifar10 of CAdam, Adam and SGD with different learning rate. X-axis is the number of epoches. The upper row is the test accuracy and the lower row is the training loss. }
% \label{fig:cifa10_lr}
% \end{figure}

% % \input{7approx.tex}


==> 8related.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\section{Related Work}

There exist two aspects of related work regarding the topic here, which are training stabilization and adaptive gradient descent.

\subsection{Stabilization}
Many efforts have been made to stabilize the training procedure of deep neural networks, including gradient clipping~\citep{bengio2013advances}, better initialization~\citep{balduzzi2017shattered,zhang2019fixup}, normalization in many machine learning problems. 

Learning rate warmup \citep{vaswani2017attention,goyal2017accurate} also serves as an important heuristics in stabilizing training procedure. Despite the lack of rigorous analysis, it has been found by experience that the warmup stage can stabilize the initial stage of training, with a high learning rate and advanced network architecture, including ResNet and Transformer. 
Recent work \citep{gotmare2018a} showed the warmup stage prevent the deeper layers from creating training instability. 

Different from previous work, we dissect the problem from the variance of the gradient statistics (i.e. adaptive learning), which is too large in the early stage of training and thus induce instability. On the other hand \citep{balduzzi2017shattered} showed the variance of the gradient of residual network keep increasing as the network become deeper and the large variance make the training  difficult. As a result, wamup and RAdam mainly focusing on fixing the deep layers, which is in consistent with \citep{gotmare2018a}.



% Our work is inspired by recent advances in  stabilizing the training procedure of deep neural network, including gradient clipping \citep{bengio2013advances}, better initialization \citep{balduzzi2017shattered,zhang2019fixup}, and normalization in many machine learning problems. 

% Learning rate warmup \citep{vaswani2017attention,goyal2017accurate} also serves as an important heuristics in stabilizing training procedure. Despite the lack of rigorous analysis, it has been found by experience that the warmup stage can stabilize the initial stage of training, with a high learning rate and advanced network architecture, including ResNet and Transformer. 
% Recent work \citep{gotmare2018a} showed the warmup stage prevent the deeper layers from creating training instability. 

% Different from previous work, we dissect the problem from the variance of the gradient statistics (i.e. adaptive learning), which is too large in the early stage of training and thus induce instability. On the other hand \citep{balduzzi2017shattered} showed the variance of the gradient of residual network keep increasing as the network become deeper and the large variance make the training  difficult. As a result, wamup and RAdam mainly focusing on fixing the deep layers, which is in consistent with \citep{gotmare2018a}.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

